A Framework of Model Reduction with Arbitrary Orders of Accuracy for the Boltzmann Equation

This paper presents a general framework for constructing reduced models that approximate the Boltzmann equation with arbitrary orders of accuracy in terms of the Knudsen number $\mathit{Kn}$, applicable to general collision models in rarefied gas dynamics. The framework is based on an orthogonal decomposition of the distribution function into components of different orders in $\mathit{Kn}$, from which the reduced models are systematically derived through asymptotic analysis. Compared to the Chapman-Enskog expansion, our approach yields more tractable model structures. Notably, we establish that a reduced model retaining all terms up to $O(\mathit{Kn}^n)$ in the expansion surprisingly yields models with order of accuracy $O(\mathit{Kn}^{n+1})$. Furthermore, when the collision term is linearized, the accuracy improves dramatically to $O(\mathit{Kn}^{2n})$. These results extend to regularized models containing second-order derivatives. As concrete applications, we explicitly derive 13-moment systems of Burnett and super-Burnett orders valid for arbitrary collision models.

==> article_Maxwell.tex <==
\subsubsection{Maxwellian iteration for the moment system}
\label{sec:Maxwell}
When Maxwellian iteration was introduced in \cite{Ikenberry1956}, the procedure was performed on the moments instead of the distribution functions as we presented in Section \ref{sec:CE}. The iteration with respect to the moments can be immediately obtained by taking the inner product of \eqref{eq:re_Maxwell_iter} and the basis functions $\varphi_{\alpha}\UP[k]$. Equivalently, we can write \eqref{eq:re_Maxwell_iter} as
\begin{displaymath}
    \pd{f_{l-1}}{t}+\bxi\cdot\nabla_{\bx}f_{l-1} = \frac{1}{\Kn} (\mL f_l + \mQs_l)
\end{displaymath}
and apply the inner product. Repeating the calculations in Section \ref{sec:deri_moment}, we have the following result:
\begin{equation}
\label{eq:moment_Max_iter}
\begin{split}
    \pd{\bdf_{l-1}^{(k)}}{t} + \left(\mbA\UP[k0] \cdot \nabla_{\bx} \bdf\UP[0] + \mB\UP[k0] \cdot \bdf\UP[0]\right) + \sum_{m=1}^{+\infty} \left(\mbA\UP[km] \cdot \nabla_{\bx} \bdf_{l-1}\UP[m] + \mB\UP[km] \cdot \bdf_{l-1}\UP[m]\right) \qquad \\
    = \frac{1}{\Kn} \sum_{m=1}^{+\infty} \mL\UP[km] \bdf_l\UP[m] + \frac{1}{\Kn} \mbQ_l\sUP[k], \quad k \geqslant 1,
\end{split}
\end{equation}
where $\bdf_l\UP[k], \mbQ_l\sUP[k]$ represent, respectively, the vectors of $f_{\alpha,l}\UP[k]$ and $\mQ_{\alpha,l}\sUP[k]$, defined by
\begin{equation}
    \label{eq:flk_Qlk}
    f_{\alpha,l}\UP[k]=\big\lg\vp_{\alpha}\UP[k],\; f_l\big\rg_{\IM},\qquad \mQ_{\alpha, l}\sUP[k]=\big\lg\vp_{\alpha}\UP[k],\; \mQs_l\big\rg_{\IM}.
\end{equation}
Note that the vector $\bdf\UP[0]$, representing the equilibrium, is not iterated, and therefore does not have a subscript denoting the index of the iteration.

It is worth pointing out that 
\begin{lemma}
    For any $l\in \bbN$, it holds $f_l\in\bbV\UP[l]$ ($\bbV\UP[l]$ defined in \eqref{eq:def_VF}).
\end{lemma}
\begin{proof}
    The proof can be completed by induction. When $l=0$, $f_0=f\UP[0]\in\bbV\UP[0]$. Suppose it holds for $0,1,\cdots,l-1$, now we consider the case of $l$. Similarly to the proof in Sec. \ref{sec:proof_thm_order}, we can derive $\pd{f_{l-1}}{t},\bxi\cdot\nabla_{\bx}{f_{l-1}},\mQs_l\in\bbF\UP[k-1]$, which yields 
    $$
    f_l=\feq+\Kn\mLd\left(\pd{f_{l-1}}{t}+\bxi\cdot\nabla_{\bx}f_{l-1}-\frac{1}{\Kn}\mQs_l\right)\in\bbV\UP[l],
    $$
    and completes the proof.
\end{proof}
This lemma directly indicates that $\bdf_l\UP[k] = 0$ for all $k > l$. Therefore, although \eqref{eq:moment_Max_iter} contains infinite series, these series are in fact finite sums due to our choice of function spaces. 

Solving $\bdf_l\UP[m]$ from \eqref{eq:moment_Max_iter} requires inverting a finite matrix, and the final conservation laws \eqref{eq:CE-conservation} that are accurate up to order $O(\Kn^n)$ can be written as
\begin{equation}
\label{eq:korder_moment}
    \pd{\bdf\UP[0]}{t}+\sum_{k=0}^n\left(\mbA\UP[0k]\cdot\nabla_{\bx}\bdf_n\UP[k]+\mB\UP[0k]\bdf_n\UP[k]\right)=0.
\end{equation}

When the Maxwellian iteration is applied to our reduced models \eqref{eq:moment_n}, the procedure can also be written in the form of \eqref{eq:moment_Max_iter}. However, due to the truncation, the infinite sums in \eqref{eq:moment_Max_iter} will become finite sums for $m$ from $1$ to $n$. Alternatively, we can write the Maxwellian iteration for \eqref{eq:moment_n} in the following form:
\begin{equation}
    \label{eq:Maxwell_l_full}
    \begin{split}
    &\pd{}{t}\begin{bmatrix}
    \bdf_{l-1}\UP[1]  \\  
    \vdots \\
    \bdf_{l-1}\UP[n] 
    \end{bmatrix} +
    \begin{bmatrix}
        \mbA\UP[10] & \mbA\UP[11] & \cdots & \mbA\UP[1n]  \\
        \vdots & \vdots & \ddots & \vdots \\
        \mbA\UP[n0] & \mbA\UP[n1] & \cdots & \mbA\UP[nn]  
    \end{bmatrix}
    \cdot \nabla_{\bx}
    \begin{bmatrix}
    \bdf\UP[0]  \\
    \bdf_{l-1}\UP[1]  \\
    \vdots  \\
    \bdf_{l-1}\UP[n]
    \end{bmatrix} +
    \begin{bmatrix}
        \mB\UP[10] & \mB\UP[11] & \cdots & \mB\UP[1n]  \\
        \vdots & \vdots & \ddots & \vdots \\
        \mB\UP[n0] & \mB\UP[n1] & \cdots & \mB\UP[nn]  
    \end{bmatrix}
    \begin{bmatrix}
    \bdf\UP[0]  \\
    \bdf_{l-1}\UP[1]  \\
    \vdots  \\
    \bdf_{l-1}\UP[n]
    \end{bmatrix} \\
    ={} &
    \frac{1}{\Kn}
    \begin{bmatrix}
        \mL\UP[11] & \ddots & \mL\UP[1n]  \\
        \ddots & \ddots & \ddots \\
        \mL\UP[n1] & \ddots & \mL\UP[nn]  
    \end{bmatrix}
    \begin{bmatrix}
    \bdf_l\UP[1]  \\
    \vdots  \\
    \bdf_l\UP[n]
    \end{bmatrix}
    +\frac{1}{\Kn}
    \begin{bmatrix}
    \mbQ_l\sUP[1]  \\
    \vdots \\
    \mbQ_l\sUP[n]
    \end{bmatrix}.
    \end{split}
\end{equation}
The resulting conservation laws still hold the form \eqref{eq:korder_moment}.

Although the iteration \eqref{eq:Maxwell_l_full} is a truncated version of \eqref{eq:moment_Max_iter}, it is not difficult to find that they are actually identical for the first $n$ iterations, due to the fact that $\bdf_l\UP[k] = 0$ when $k > l$. Therefore, by Definition \ref{def:OOA}, the reduced model \eqref{eq:moment_n} has an order of accuracy greater than or equal to $n$. The actual order of accuracy has been provided in Theorems \ref{thm:full} and \ref{thm:linear}, whose proofs will be detailed in the following subsections. 

==> article_full.tex <==
\subsubsection{The full moment system}
\label{sec:full_order}
Denoting the result after $l$ iterations of $f\UP[k]$ as $f\UP[k]_l$, which can be computed by $f\UP[k]_l=\mP_{\bbV\UP[k]\cap\left(\bbV\UP[k-1]\right)^{\perp}}f_l$, where $f_l$ is iterated from \eqref{eq:re_Maxwell_iter}. Besides, from the definition of $\bbV\UP[l]$ in \eqref{eq:def_VF}, it can be easily inducted that $f_{l}\in\bbV\UP[l]$. This indicates $f\UP[k]_l=0, k>l$, and
\begin{equation}
    \label{eq:exp_Max_fk}
    f_l=\sum_{k=0}^{\infty}f\UP[k]_l=\sum_{k=0}^{l}f\UP[k]_l.
\end{equation}

In this section, we consider the general system with quadratic collision operator. Firstly, we need to confirm the approximation order of truncation \eqref{eq:def_tQ}. The result is displayed in the following lemma:
\begin{lemma}
    \label{lemma:approx_Q}
    For $\mQs_l$ defined in \eqref{eq:def_mQs_l}, it holds
    \begin{equation}
        \label{eq:approx_mQs_l}
        \mQs_l=\sum_{\substack{i,j\geqslant 1 \\i+j\leqslant l}}\mQ[f\UP[i],f\UP[j]]+O(\Kn^{l+1}).
    \end{equation}
\end{lemma}
\begin{proof}
    With \eqref{eq:exp_Max_fk}, we can simplify \eqref{eq:def_mQs_l} as
    \begin{equation}
        \label{eq:simp_mQs_1}
        \begin{split}
            \mQs_l&=\sum_{\substack{r,s\geqslant 1 \\r+s\leqslant l}}\mQ[f_r-f_{r-1}, f_s-f_{s-1}] 
            =\sum_{r=1}^{l-1}\mQ[f_r-f_{r-1}, f_{l-r}-f_0] \\
            &=\sum_{r=1}^{l-1}\sum_{i=1}^r\sum_{j=1}^{l-r}\mQ[f_r\UP[i]-f_{r-1}\UP[i], f_{l-r}\UP[j]] 
            =\sum_{r=1}^{l-1}\sum_{i=1}^r\sum_{j=1}^{l-r}\mQ[f_r\UP[i]-f_{r-1}\UP[i], f\UP[j]]+O(\Kn^{l+1}) \\
            &=\sum_{\substack{i,j\geqslant 1 \\i+j\leqslant l}}\sum_{r=i}^{l-j}\mQ[f_r\UP[i]-f_{r-1}\UP[i], f\UP[j]]+O(\Kn^{l+1}) \\
            &=\sum_{\substack{i,j\geqslant 1 \\i+j\leqslant l}}\mQ[f_{l-j}\UP[i],f\UP[j]]+O(\Kn^{l+1}) 
            =\sum_{\substack{i,j\geqslant 1 \\i+j\leqslant l}}\mQ[f\UP[i],f\UP[j]]+O(\Kn^{l+1}),
        \end{split}
    \end{equation}
    where the fourth equality utilizes $f_r\UP[i]-f_{r-1}\UP[i]=O(\Kn^r),\;f\UP[j]=f_{l-r}\UP[j]+O(\Kn^{l-r+1})$, and the last equality utilizes $f\UP[i]=f_{l-r}\UP[i]+O(\Kn^{l-r+1}),\; f\UP[j]=O(\Kn^j)$.
\end{proof}

Lemma \ref{lemma:approx_Q} indicates that for the truncation in \eqref{eq:def_tQ}, it holds
\begin{equation}
    \label{eq:approx_Q}
    \qquad \mbQ\sUP[k]=\mbQ\sUP[k]_{n+1}+O(\Kn^{n+2}).
\end{equation}

Then, we present the proof of Thm. \ref{thm:full} as below:

\begin{proof}
    We adopt the notations and the definitions (such as $\mFT, \mFA, \mFC, \mFL$) as in Sec. \ref{sec:lin_order}. 
    The system with approximation order $O(\Kn^{n+1})$ can be formulated as
    \begin{equation}
        \label{eq:full_approx_np1}
        \pd{\bdf\UP[0]}{t}+\mbA_0\UP[00]\cdot \nabla_{\bx}\bdf\UP[0]+\mFA(0,n+1,0)+\mC_0\UP[00]\bdf\UP[0]+\mFC(0,n+1,0)=0.
    \end{equation}

    In the system with full collision operator, \eqref{eq:Max_mF} becomes
    \begin{equation}
        \label{eq:Max_mF_full}
        \begin{split}
            \mFL(i,k,l)=\Kn\Bigg[&\pd{}{t}\mFT(i,k-1,l)+\nabla_{\bx}\cdot\left(\mbA_l\UP[i0]\bdf\UP[0]\right)+\nabla_{\bx}\cdot\mFA(i,k-1,l)\\
            &+\mC_l\UP[i0]\bdf\UP[0]+\mFC(i,k-1,l)\Bigg]-\mbQ_k\sUP[i].
        \end{split}
    \end{equation}    
    Since $\mbQ\sUP[0]=0$, the Maxwellian iteration is identical to the linearized case in the first step. Thus, the relationships \eqref{eq:rela_mFTl0}-\eqref{eq:rela_mFCl0} still hold for $i=0$.
    Consequently, $\mFA(0,n+1,0)$ and $\mFC(0,n+1,0)$ can be replaced by
    \begin{equation}
        \label{eq:recur_mFA_full}
        \begin{split}
            \mFA(0,n+1,0)=&\Kn\left(\mbA_0\UP[10]\right)^T\left(\mL_{0}\UP[11]\right)^{-1}
            \Bigg[\pd{}{t}\mFT(1,n,0)+\nabla_{\bx}\cdot\left(\mbA_0\UP[10]\bdf\UP[0]\right)\\
            &+\nabla_{\bx}\cdot\mFA(1,n,0)      
            +\mC_0\UP[10]\bdf\UP[0]+\mFC(1,n,0)\Bigg]-\left(\mbA_0\UP[10]\right)^T\left(\mL_{0}\UP[11]\right)^{-1}\mbQ_{n+1}\sUP[1], 
        \end{split}
    \end{equation}
    and
    \begin{equation}
        \label{eq:recur_mFC_full}
        \begin{split}
            \mFC(0,n+1,0)=&\Kn\left(\mB_0\UP[10]\right)^T\left(\mL_{0}\UP[11]\right)^{-1}
            \Bigg[\pd{}{t}\mFT(1,n,0)+\nabla_{\bx}\cdot\left(\mbA_0\UP[10]\bdf\UP[0]\right)\\
            &+\nabla_{\bx}\cdot\mFA(1,n,0)      
            +\mC_0\UP[10]\bdf\UP[0]+\mFC(1,n,0)\Bigg]-\left(\mB_0\UP[10]\right)^T\left(\mL_{0}\UP[11]\right)^{-1}\mbQ_{n+1}\sUP[1].
        \end{split}
    \end{equation}
Some facts can be observed:
\begin{itemize}
    \item All the matrices on the right-hand side of \eqref{eq:recur_mFA_full} and \eqref{eq:recur_mFC_full} can be directly extracted from the truncated system \eqref{eq:moment_n}.
    \item Since $\mbQ\sUP[k]=\mbQ\sUP[k]_{n+1}+O(\Kn^{n+2})=\mbQ_{n}\sUP[k]+O(\Kn^{n+1})$, the results of $f_n$ can be accurately obtained with $n$ times of Maxwellian iterations from \eqref{eq:moment_n}. This is to say, the terms of $\mFT(1,n,0)$, $\mFA(1,n,0)$ and $\mFC(1,n,0)$ can be accurately computed.
    \item Since $\mbQ\sUP[1]=\mbQ\sUP[1]_{n+1}+O(\Kn^{n+2})$, the moment system \eqref{eq:moment_n} can provide an approximation of $\mbQ_{n+1}\sUP[1]$ with order $O(\Kn^{n+2})$.
\end{itemize}
Combining these facts, we know that $\mFA(0,n+1,0)$ and $\mFC(0,n+1,0)$ can be approximated with order $O(\Kn^{2n+2})$ from moment model \eqref{eq:moment_n}, which verifies its order of $O(\Kn^{n+1})$. 
\end{proof}

\begin{remark}
    \label{rmk:terms}
    For $n\geqslant 2$, the terms $\pd{\bdf\UP[n]}{t}$ and matrices $\mbA\UP[in], \mB\UP[in], 2\leqslant i\leqslant n$ are not involved in the ultimate expression, which can be set as $0$ while the system maintains the approximation order of $O(\Kn^{n+1})$. Besides, the truncation of collision term can be modified to
    \begin{equation}
        \label{eq:modify_trun_Q}
        \begin{split}
            &\widetilde{\mQ}_{\alpha}\sUP[1]=\sum_{l=1}^{n} \sum_{m=1}^{n+1-l}\mQ[f\UP[l],f\UP[m]], \\
            &\widetilde{\mQ}_{\alpha}\sUP[k]=\sum_{l=1}^{n-1} \sum_{m=1}^{n-l}\mQ[f\UP[l],f\UP[m]], \quad k\geqslant2,
        \end{split}
    \end{equation}
    which also does not affect the asymptotic order.
\end{remark}

Thm. \ref{thm:full} requires particular approximation order of $\mbQ\sUP[k]$. The following lemma provides the approach to approximate $\mQs_l$ with order $O(\Kn^l)$:

Consequently, the quadratic term in \eqref{eq:moment_n} can be truncated as 
% \begin{equation}
%     \label{eq:Q_moment_n}
%     \begin{split}
%         &\mbQ\sUP[0]=0, \\
%         &\mbQ\sUP[1]=\mP_{\bbV\UP[1]\cap \left(\bbV\UP[0]\right)^{\perp}}\sum_{\substack{i,j\geqslant 1 \\i+j\leqslant n+1}}\mQ[f\UP[i],f\UP[j]], \\
%         &\mbQ\sUP[k]=\mP_{\bbV\UP[k]\cap \left(\bbV\UP[k-1]\right)^{\perp}}\sum_{\substack{i,j\geqslant 1 \\i+j\leqslant n}}\mQ[f\UP[i],f\UP[j]],\quad k\geqslant 2.
%     \end{split}
% \end{equation}
It keeps the system closed with $f\UP[0], \cdots, f\UP[n]$, and also has the approximation order of $O(\Kn^{n+1})$.

As an application, we briefly verify the super-Burnett order of \eqref{eq:13-moment_super_Burnett} in the following. Letting $n=2$ in Thm. \ref{thm:full}, the terms involved in \eqref{eq:recur_mFA_full} and \eqref{eq:recur_mFC_full} are
\begin{equation}
    \label{eq:term_super_Burnett}
    \mFT(1,2,0),\quad \mFA(1,2,0),\quad \mFC(1,2,0),\quad \mbQ_3\sUP[1]
\end{equation}

The results of $f_2$ is required from the Maxwellian iteration, which can be obtained by
\begin{equation}
    \label{eq:Maxwell_full_2}
    \begin{split}
    &\pd{}{t}\left[
    \begin{array}{c}
    \bdf_{l-1}\UP[1]  \\
    0
    \end{array}
    \right]+
    \left[
    \begin{array}{cc}
        \mbA\UP[10] & \mbA\UP[11] \\
        \mbA\UP[20] & \mbA\UP[21] 
    \end{array}
    \right]
    \cdot \nabla_{\bx}\left[
    \begin{array}{c}
    \bdf_{l-1}\UP[1]  \\
    0
    \end{array}
    \right]+
    \left[
    \begin{array}{cc}
        \mB\UP[10] & \mB\UP[11] \\
        \mB\UP[20] & \mB\UP[21] 
    \end{array}
    \right]\left[
    \begin{array}{c}
    \bdf_{l-1}\UP[1]  \\
    0
    \end{array}
    \right]\\
    =&
    \frac{1}{\Kn}
    \left[
    \begin{array}{cc}
        \mL\UP[11] & \mL\UP[12] \\
        \mL\UP[21] & \mL\UP[22] 
    \end{array}
    \right]\left[
    \begin{array}{c}
    \bdf_l\UP[1]  \\
    \bdf_l\UP[2]
    \end{array}
    \right]+\frac{1}{\Kn}
    \left[
    \begin{array}{c}
    \mbQ_l\sUP[1]  \\
    \mbQ_l\sUP[2]
    \end{array}
    \right],\quad l=1,2.
    \end{split}
\end{equation}
This is fully covered by system \eqref{eq:13-moment_super_Burnett}. Besides, the matrices are also included in the system, which validates that \eqref{eq:13-moment_super_Burnett} exhibits the super-Burnett approximation order.


\begin{remark}
    Currently, we have not found a method to further simplify the quadratic term in \eqref{eq:recur_mFA_full} and \eqref{eq:recur_mFC_full}. 
    Comparing Thm. \ref{thm:linear} and Thm. \ref{thm:full}, it can be observed the linearized part of \eqref{eq:moment_n} can exhibit the accuracy order of $O(\Kn^{2n})$, while the quadratic part only has $O(\Kn^{n+1})$. In some situations, the quadratic collision only has a small impact, and the model may have better approximation effect.  
\end{remark}

==> article_linear.tex <==
\subsubsection{The system with linearized collision operator}
\label{sec:lin_order}

We first study the linearized case with $\mbQ\sUP[k] = 0$ in \eqref{eq:moment_n} and $\mbQ_l\sUP[k] = 0$ in \eqref{eq:Maxwell_l_full}.
Before studying the approximation order of \eqref{eq:lin_moment_n}, we need to explore some properties of the matrix $\mbA$, $\mB$ and $\mL$ from the Maxwellian iteration. 

From \eqref{eq:re_Maxwell_iter}, it can be seen that $\mP_{\bbV\UP[0]}f_l=\feq=f\UP[0]$, which yields $f_l\UP[0]=f\UP[0]$.
The Maxwellian iteration of step $l$ has the form 
\begin{equation}
    \label{eq:lin_moment_Max}
    \begin{split}
    &\pd{}{t}\left[
    \begin{array}{c}
    \bdf\UP[0]  \\  
    \bdf\UP[1]_{l-1} \\
    \vdots \\
    \bdf\UP[n]_{l-1}
    \end{array}
    \right]+
    \left[
    \begin{array}{ccc}
        \mbA\UP[00] & \ddots & \mbA\UP[0n]  \\
        \ddots & \ddots & \ddots \\
        \mbA\UP[n0] & \ddots & \mbA\UP[nn]  
    \end{array}
    \right]
    \cdot \nabla_{\bx}\left[
    \begin{array}{c}
    \bdf\UP[0]  \\
    \bdf\UP[1]_{l-1} \\
    \vdots  \\
    \bdf\UP[n]_{l-1} 
    \end{array}
    \right]\\
    &+
    \left[
    \begin{array}{ccc}
        \mB\UP[00] & \ddots & \mB\UP[0n]  \\
        \ddots & \ddots & \ddots \\
        \mB\UP[n0] & \ddots & \mB\UP[nn]  
    \end{array}
    \right]\left[
    \begin{array}{c}
    \bdf\UP[0]  \\
    \bdf\UP[1]_{l-1} \\
    \vdots  \\
    \bdf\UP[n]_{l-1} 
    \end{array}
    \right]=
    \frac{1}{\Kn}
    \left[
    \begin{array}{ccc}
        \mL\UP[00] & \ddots & \mL\UP[0n]  \\
        \ddots & \ddots & \ddots \\
        \mL\UP[n0] & \ddots & \mL\UP[nn]  
    \end{array}
    \right]\left[
    \begin{array}{c}
    \bdf\UP[0]  \\
    \bdf\UP[1]_{l} \\
    \vdots  \\
    \bdf\UP[n]_{l} 
    \end{array}
    \right].
    \end{split}
\end{equation}
Firstly, since $\mL\UP[i0]=0, \mL\UP[0j]=0$, the equations of $\pd{\bdf\UP[0]}{t}$ in \eqref{eq:lin_moment_Max} will not affect the results of Maxwellian iteration, which will be omitted in the following derivations. 

% Setting $l=1$ and utilizing the fact that $f_l\UP[k]=0,\; k>l$, we can simplify \eqref{eq:lin_moment_Max} as
% \begin{equation}
%     \label{eq:lin_Max_l1}
%     \left[
%     \begin{array}{c}
%         \mbA\UP[10]  \\
%         \mbA\UP[20]  \\ 
%         \vdots \\ 
%         \mbA\UP[n0]
%     \end{array}
%     \right]
%     \cdot 
%     \nabla_{\bx}\bdf\UP[0]=
%     \frac{1}{\Kn}
%     \left[
%     \begin{array}{c}
%         \mL\UP[11] \\
%         \mL\UP[21] \\
%         \vdots \\
%         \mL\UP[n1]  
%     \end{array}
%     \right]\bdf\UP[1]_1.
% \end{equation}
% By Gaussian elimination, \eqref{eq:lin_Max_l1} can be transformed into
% \begin{equation}
%     \label{eq:lin_Max_l1_2}
%     \left[
%     \begin{array}{c}
%         \mbA\UP[10]  \\
%         \mbA\UP[20]-\mL\UP[21]\left(\mL\UP[11]\right)^{-1}\mbA\UP[10]  \\ 
%         \vdots \\ 
%         \mbA\UP[n0]-\mL\UP[n1]\left(\mL\UP[11]\right)^{-1}\mbA\UP[10]
%     \end{array}
%     \right]
%     \cdot 
%     \nabla_{\bx}\bdf\UP[0]=
%     \frac{1}{\Kn}
%     \left[
%     \begin{array}{c}
%         \mL\UP[11] \\
%         0 \\
%         \vdots \\
%         0
%     \end{array}
%     \right]\bdf\UP[1]_1,
% \end{equation}
% which yields
% \begin{equation}
%     \label{eq:rela_AL_l1}
%     \mbA\UP[i0]=\mL\UP[i1]\left(\mL\UP[11]\right)^{-1}\mbA\UP[10],\quad i\geqslant 1,
% \end{equation}
% and 
% \begin{equation}
%     \label{eq:result_f1_l1}
%     \bdf_1\UP[1]=\Kn \left(\mL\UP[11]\right)^{-1}\mbA\UP[10]\cdot\nabla_{\bx}\bdf\UP[0].
% \end{equation}
% Setting $l=2$ and retaining the non-zero terms, the second-step iteration can be expressed as
% \begin{equation}
%     \label{eq:lin_Max_l2}
%     \pd{}{t}\left[
%     \begin{array}{c}
%         \bdf_1\UP[1] \\
%         0  \\ 
%         \vdots \\ 
%         0
%     \end{array}
%     \right]+
%     \left[
%     \begin{array}{cc}
%         \mbA\UP[10] & \mbA\UP[11] \\
%         \mbA\UP[20] & \mbA\UP[21] \\ 
%         \vdots & \vdots \\ 
%         \mbA\UP[n0] & \mbA\UP[n1] 
%     \end{array}
%     \right]\cdot \nabla_{\bx}\left[ 
%     \begin{array}{c}
%          \bdf\UP[0]  \\
%          \bdf\UP[1]_1  
%     \end{array}
%     \right]=
%     \frac{1}{\Kn}\left[
%     \begin{array}{cc}
%         \mL\UP[11] & \mL\UP[12]  \\
%         \mL\UP[21] & \mL\UP[22]  \\ 
%         \vdots & \vdots \\ 
%         \mL\UP[n1] & \mL\UP[n2]
%     \end{array}
%     \right]\left[ 
%     \begin{array}{c}
%          \bdf\UP[1]_2  \\
%          \bdf\UP[2]_2  
%     \end{array}
%     \right].
% \end{equation}
% To solve $\bdf\UP[1]_2$ and $\bdf\UP[2]_2$, we can again apply the Gaussian elimination, which leads to
% \begin{equation}
%     \label{eq:lin_Max_l2_Gauss}
%     \left[
%     \begin{array}{c}
%         I \\
%         \mT_1\UP[21]  \\ 
%         \vdots \\ 
%         \mT_1\UP[n1]
%     \end{array}
%     \right]\pd{\bdf_1\UP[1]}{t}+
%     \left[
%     \begin{array}{cc}
%         \mbA\UP[10] & \mbA\UP[11] \\
%         0 & \mbA_1\UP[21] \\ 
%         \vdots & \vdots \\ 
%         0 & \mbA_1\UP[n1] 
%     \end{array}
%     \right]\cdot \nabla_{\bx}\left[ 
%     \begin{array}{c}
%          \bdf\UP[0]  \\
%          \bdf\UP[1]_1  
%     \end{array}
%     \right]=
%     \frac{1}{\Kn}\left[
%     \begin{array}{cc}
%         \mL\UP[11] & \mL\UP[12]  \\
%         0 & \mL_1\UP[22]  \\ 
%         \vdots & \vdots \\ 
%         0 & \mL_1\UP[n2]
%     \end{array}
%     \right]\left[ 
%     \begin{array}{c}
%          \bdf\UP[1]_2  \\
%          \bdf\UP[2]_2  
%     \end{array}
%     \right],
% \end{equation}
% where $I$ is the identity matrix, and 
% \begin{equation}
%     \label{eq:lin_def_TAL1}
%     \begin{split}
%        &\mT_1\UP[i1]=-\mL\UP[i1]\left(\mL\UP[11]\right)^{-1}, \quad 
%        \mbA_1\UP[i1]=\mbA\UP[k1]-\mL\UP[i1]\left(\mL\UP[11]\right)^{-1}\mbA\UP[11], \\
%        &\mL_1\UP[i2]=\mL\UP[i2]-\mL\UP[i1]\left(\mL\UP[11]\right)^{-1}\mL\UP[12], \quad i\geqslant2.
%     \end{split}
% \end{equation}
% Consequently, the form of \eqref{eq:lin_Max_l2_Gauss} allows us to solve $\bdf\UP[2]_2$ firstly, and then solve $\bdf\UP[1]_2$ from the first row. In fact, this Gaussian elimination can decouple the terms of $\bdf\UP[1]_l$ in the $l$-th Maxwellian iteration for $l\geqslant 2$. Similarly, the terms of $\bdf\UP[2]_l, \bdf\UP[3]_l, \cdots$ can also be decoupled in this way. Details will be revealed in the following.

\paragraph{General framework of the Maxwellian iteration}
For $l\geqslant 0$, we define the matrices: 
\begin{equation}
    \label{eq:lin_def_TABL_l}
    \begin{split}
        &\mT_0\UP[ij]=\mT\UP[ij]\triangleq\delta_{ij}I,\quad \mbA_0\UP[ij]=\mbA\UP[ij], \quad \mB_0\UP[ij]=\mB\UP[ij], \quad \mL_0\UP[ij]=\mL\UP[ij], \\
        &\mT_l\UP[ij]=\left\{
        \begin{array}{ll}
            \mT_{l-1}\UP[ij]-\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\mT_{l-1}\UP[lj],  & i>l; \\ %,\; l\leqslant j;  \\
            \mT_{l-1}\UP[ij], & \text{otherwise},
        \end{array}\right. \\
        &\mbA_l\UP[ij]=\left\{
        \begin{array}{ll}
            \mbA_{l-1}\UP[ij]-\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\mbA_{l-1}\UP[lj],  & i>l; \\ %,\; l\leqslant j+1;  \\
            \mbA_{l-1}\UP[ij], & \text{otherwise},
        \end{array}\right. \\
        &\mB_l\UP[ij]=\left\{
        \begin{array}{ll}
            \mB_{l-1}\UP[ij]-\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\mB_{l-1}\UP[lj],  & i>l; \\ %,\; l\leqslant j;  \\
            \mB_{l-1}\UP[ij], & \text{otherwise},
        \end{array}\right. \\
        &\mL_l\UP[ij]=\left\{
        \begin{array}{ll}
            \mL_{l-1}\UP[ij]-\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\mL_{l-1}\UP[lj],  & i>l; \\ %,\; l\leqslant j;  \\
            \mL_{l-1}\UP[ij], & \text{otherwise}.
        \end{array}\right. \\
    \end{split}
\end{equation}

\begin{lemma}
\label{lemma:Max_Gauss}
For any $l\geqslant 0$, it holds that 
\begin{enumerate}
    \item $\mL_l\UP[ij]=0$ when $j\leqslant i-1$ and $j\leqslant l$, \label{state:L0}
    \item $\mbA_l\UP[ij]=0$, $\mB_l\UP[ij]=0$, $\mT_l\UP[ij]=0$ when $j\leqslant i-2$ and $j \leqslant l-1$, \label{state:ABT0}
    \item $\left(\mL_l\UP[ij]\right)^T=\mL_l\UP[ji]$ when $i>l$ and $j>l$, \label{state:sym_L}
    \item Omitting the equation of $\pd{\bdf\UP[0]}{t}$, the linearized moment system \eqref{eq:moment_n} with $\mbQ\sUP[k] = 0$ is equivalent to \label{state:Maxwell_l}
\begin{equation}
    \label{eq:lin_Max_gen_l}
    \begin{split}
    &\left[
    \begin{array}{ccc}
        \mT_{l}\UP[11] & \ddots & \mT_{l}\UP[1n]  \\
        \ddots & \ddots & \ddots \\ 
        \mT_{l}\UP[n1] & \ddots & \mT_{l}\UP[nn]  
    \end{array}
    \right]
    \pd{}{t}
    \left[
    \begin{array}{c}
         \bdf\UP[1] \\
         \vdots \\ 
         \bdf\UP[n]
    \end{array}
    \right]+
    \left[
    \begin{array}{ccc}
        \mbA_{l}\UP[10] & \ddots & \mbA_{l}\UP[1n]  \\
        \ddots & \ddots & \ddots \\ 
        \mbA_{l}\UP[n0] & \ddots & \mbA_{l}\UP[nn] 
    \end{array}
    \right]\cdot\nabla_{\bx}
    \left[
    \begin{array}{c}
        \bdf\UP[0]  \\
        \bdf\UP[1] \\ 
        \vdots \\ 
        \bdf\UP[n] 
    \end{array}
    \right] \\
    &+\left[
    \begin{array}{ccc}
        \mB_l\UP[10] & \ddots & \mB_l\UP[1n]  \\
        \ddots & \ddots & \ddots \\
        \mB_l\UP[n0] & \ddots & \mB_l\UP[nn]  
    \end{array}
    \right]\left[
    \begin{array}{c}
    \bdf\UP[0]  \\
    \vdots  \\
    \bdf\UP[n]
    \end{array}
    \right]
    =\frac{1}{\Kn}\left[ 
    \begin{array}{ccc}
        \mL_{l}\UP[11] & \ddots & \mL_{l}\UP[1n]  \\
        \ddots & \ddots & \ddots \\
        \mL_{l}\UP[n1] & \ddots & \mL_{l}\UP[nn]
    \end{array}
    \right]\left[
    \begin{array}{c}
         \bdf\UP[1] \\
         \vdots \\ 
         \bdf\UP[n]
    \end{array}
    \right].
    \end{split}
\end{equation}
\end{enumerate}
\end{lemma}
\begin{proof}
    Statement \ref{state:L0} can be directly observed from \eqref{eq:lin_def_TABL_l}. 
    
    Statement \ref{state:Maxwell_l} can be verified with the Gaussian elimination on \eqref{eq:moment_n}. When $l=0$, it corresponds to the original system after omitting the first row. Now suppose we have derived the system of subscript $l-1$. For $i>l$, we multiply $-\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}$ to the $l$-th row, and then add the result to the $i$-th row. From the definition of $\mL_l\UP[ij]$, the system of subscript $l-1$ will be equivalently transformed to the system of subscript $l$, which proves state \ref{state:Maxwell_l} by induction.

    Statement \ref{state:ABT0} can also be proved with induction. When $l=0$, it is naturally satisfied. Suppose it holds for $l-1$, now we consider the case of $l$. When $j\leqslant l-2$ and $j\leqslant i-2$, from the induction hypothesis, we have $\mT_{l-1}\UP[ij]=0, \mT_{l-1}\UP[lj]=0$, which yields $\mT\UP[ij]_l=0$ by definition \eqref{eq:lin_def_TABL_l}. Similarly, it can be obtained that $\mbA\UP[ij]_l=0$ and $\mB\UP[ij]_l=0$.
    When $j=l-1$, we consider the Maxwellian iteration of step $l$. Eliminating the zero terms of $f_l\UP[k], k>l$, the rows beginning from $l$ can be written as
    \begin{equation}
        \label{eq:lin_Max_l2n}
        \left[
    \begin{array}{c}
        \mT_l\UP[l,l-1]  \\ 
        \vdots \\ 
        \mT_l\UP[n,l-1]
    \end{array}
    \right]\pd{\bdf_{l-1}\UP[l-1]}{t}+
    \left[
    \begin{array}{c}
        \mbA_l\UP[l,l-1] \\
        \vdots \\ 
        \mbA_l\UP[n,l-1] 
    \end{array}
    \right]\cdot \nabla_{\bx}\bdf_{l-1}\UP[l-1]
    +\left[
    \begin{array}{c}
        \mB_l\UP[l,l-1] \\
        \vdots \\ 
        \mB_l\UP[n,l-1] 
    \end{array}
    \right]\bdf_{l-1}\UP[l-1]
    =\frac{1}{\Kn}\left[
    \begin{array}{c}
         \mL_l\UP[ll]  \\
         \vdots \\ 
         \mL_l\UP[nl]
    \end{array}
    \right]\bdf_{l}\UP[l],
\end{equation}
where the columns $0$ to $l-2$ vanish due to the first state and the induction. Since $\mL_{l}\UP[il]=0$ for $i=l+1, \cdots, n$, one can obtain 
$$\mT_l\UP[i,l-1]\pd{\bdf_{l-1}\UP[l-1]}{t}+\mbA_l\UP[i,l-1]\cdot\nabla_{\bx}\bdf_{l-1}\UP[l-1]+\mB_l\UP[i,l-1]\bdf_{l-1}\UP[l-1]=0,\quad i=l+1,\cdots,n.$$
\lyx{Seems $\mLd$ is tridiagonal! (because of the definition of $\bbV\UP[k]$) Let me check it.}
This yields $\mT_l\UP[i, l-1]=0, \mbA_l\UP[i, l-1]=0, \mB_l\UP[i, l-1]=0$ for $i=l+1, \cdots, n$ and completes the induction of the state \ref{state:ABT0}. 

Since $\mL$ is symmetric, state \ref{state:sym_L} holds for $l=0$. For $l>0$, it can be easily verified by induction from the definition \eqref{eq:lin_def_TABL_l}. 
\end{proof}
\begin{corollary}
    \label{coro:rela_A}
    For $i>l$, it holds 
    \begin{equation}
        \label{eq:coro_A}
        \mbA_l\UP[il]=\mL_l\UP[i, l+1]\left(\mL_l\UP[l+1, l+1]\right)^{-1} \mbA_l\UP[l+1, l].
    \end{equation}
\end{corollary}
\begin{proof}
    When $i=l+1$, it can be observed straightforwardly. When $i\geqslant l+2$, from \eqref{eq:lin_def_TABL_l} and Lemma \ref{lemma:Max_Gauss}, one has 
    \begin{equation}
        \label{eq:proof_coro_A}
        \mbA_l\UP[il]-\mL_l\UP[i, l+1]\left(\mL_l\UP[l+1, l+1]\right)^{-1} \mbA_l\UP[l+1, l]=\mbA_{l+1}\UP[il]=0,
    \end{equation}
    which completes the proof.
\end{proof}

\begin{lemma}
    \label{lemma:exp_A_0ij}
    For $i\geqslant 1, j\geqslant 0$, it holds  
    \begin{equation}
        \label{eq:exp_A_0ij_trans}
        \left(\mbA_0\UP[ij]\right)^T=\sum_{l=1}^{j+1}\left(\mbA_{l-1}\UP[lj]\right)^T\left(\mL_{l-1}\UP[ll]\right)^{-1}\mL_{l-1}\UP[li].
    \end{equation}
\end{lemma}
Proof of Lemma \ref{lemma:exp_A_0ij} can be found in App. \ref{app:proof_lemma_A_0ij}. It naturally follows that
\begin{equation}
    \label{eq:exp_A_0ij}
    \mbA_0\UP[ij]=\left(\mbA_0\UP[ji]\right)^T=\sum_{l=1}^{i+1}\left(\mbA_{l-1}\UP[li]\right)^T\left(\mL_{l-1}\UP[ll]\right)^{-1}\mL_{l-1}\UP[lj].
\end{equation}
Similarly, it can be verified that
\begin{align}
    \label{eq:coro_B}
    &\mB_l\UP[il]=\mL_l\UP[i,l+1]\left(\mL_l\UP[l+1,l+1]\right)^{-1}\mB_l\UP[l+1,l],\quad i>l, \\
    \label{eq:coro_T}
    &\mT_l\UP[il]=\mL_l\UP[i,l+1]\left(\mL_l\UP[l+1,l+1]\right)^{-1}\mT_l\UP[l+1,l],\quad i>l,
\end{align}
and
\begin{align}
    \label{eq:exp_B_0ij}
    &\left(\mB_0\UP[ji]\right)^T=\sum_{l=1}^{i+1}\left(\mB_{l-1}\UP[li]\right)^T\left(\mL_{l-1}\UP[ll]\right)^{-1}\mL_{l-1}\UP[lj], \\
    \label{eq:exp_T_0ij}
    &\mT_0\UP[ij]=\left(\mT_0\UP[ji]\right)^T=\sum_{l=1}^{i+1}\left(\mT_{l-1}\UP[li]\right)^T\left(\mL_{l-1}\UP[ll]\right)^{-1}\mL_{l-1}\UP[lj].
\end{align}
% Since $\mbA$ and $\mL$ are both symmetric, it follows that
% \begin{equation}
%     \label{eq:coro_A_trans}
    
% \end{equation}
We define 
\begin{equation}
    \label{eq:def_C}
    \mC_l\UP[ij]=\pd{}{t}\mT_l\UP[ij]+\nabla_{\bx}\cdot\mA_l\UP[ij]-\mB_l\UP[ij],\quad \mC\UP[ij]=\mC_0\UP[ij],
\end{equation}
then the moment system \eqref{eq:lin_Max_gen_l} is equivalent to
\begin{equation}
    \label{eq:lin_moment_C}
    \begin{split}
    &\pd{}{t}\left[
    \begin{array}{ccc}
        \mT_{l}\UP[11] & \ddots & \mT_{l}\UP[1n]  \\
        \ddots & \ddots & \ddots \\ 
        \mT_{l}\UP[n1] & \ddots & \mT_{l}\UP[nn]  
    \end{array}
    \right]\left[
    \begin{array}{c}
    \bdf\UP[0]  \\  
    \bdf\UP[1] \\
    \vdots \\
    \bdf\UP[n]
    \end{array}
    \right]+\nabla_{\bx}\cdot
    \left[
    \begin{array}{ccc}
        \mbA_{l}\UP[10] & \ddots & \mbA_{l}\UP[1n]  \\
        \ddots & \ddots & \ddots \\ 
        \mbA_{l}\UP[n0] & \ddots & \mbA_{l}\UP[nn] 
    \end{array}
    \right]
    \left[
    \begin{array}{c}
        \bdf\UP[0]  \\
        \bdf\UP[1] \\ 
        \vdots \\ 
        \bdf\UP[n] 
    \end{array}
    \right] \\
    &-\left[
    \begin{array}{ccc}
        \mC_l\UP[10] & \ddots & \mC_l\UP[1n]  \\
        \ddots & \ddots & \ddots \\
        \mC_l\UP[n0] & \ddots & \mC_l\UP[nn]  
    \end{array}
    \right]\left[
    \begin{array}{c}
    \bdf\UP[0]  \\
    \vdots  \\
    \bdf\UP[n]
    \end{array}
    \right]
    =\frac{1}{\Kn}\left[ 
    \begin{array}{ccc}
        \mL_{l}\UP[11] & \ddots & \mL_{l}\UP[1n]  \\
        \ddots & \ddots & \ddots \\
        \mL_{l}\UP[n1] & \ddots & \mL_{l}\UP[nn]
    \end{array}
    \right]\left[
    \begin{array}{c}
         \bdf\UP[1] \\
         \vdots \\ 
         \bdf\UP[n]
    \end{array}
    \right].
    \end{split}
\end{equation}

When $l=0$, the component of $\mC\UP[ij]$ can be computed as
\begin{equation}
    \label{eq:comp_C0}
    \begin{split}
        C_{\alpha,\beta}\UP[ij]&=\pd{}{t}T_{\alpha,\beta}\UP[ij]+\nabla_{\bx}\cdot\bA_{\alpha,\beta}\UP[ij]-B_{\alpha,\beta}\UP[ij]\\
        &=\pd{}{t}\left\lg\vp_{\beta}\UP[l], \vp_{\alpha}\UP[k] \right\rg_{\IM}+\nabla_{\bx}\cdot\left\lg\bxi\vp_{\beta}\UP[l], \vp_{\alpha}\UP[k] \right\rg_{\IM}-\left\lg\pd{\vp_{\beta}\UP[l]}{t}+\bxi\cdot\nabla_{\bx}\vp_{\beta}\UP[l], \vp_{\alpha}\UP[k] \right\rg_{\IM} \\
        &=\left\lg\vp_{\beta}\UP[l], \pd{\vp_{\alpha}\UP[k]}{t}+\bxi\cdot\nabla_{\bx}\vp_{\alpha}\UP[k] \right\rg_{\IM}\\
        &=B_{\beta,\alpha}\UP[ji],
    \end{split}
\end{equation}
which indicates
\begin{equation}
    \label{eq:exp_C_0ij}
    \mC_0\UP[ij]=\left(\mB_0\UP[ji]\right)^T=\sum_{l=1}^{i+1}\left(\mB_{l-1}\UP[li]\right)^T\left(\mL_{l-1}\UP[ll]\right)^{-1}\mL_{l-1}\UP[lj].
\end{equation}

\paragraph{Conclusions of approximation order}
The expressions $\mFT, \mFA, \mFC, \mFL$ are defined as
% \begin{align}
%     \label{eq:def_mF_T}
%     &\mFT(i,k,l)=\sum_{j=1}^k\mT_{l}\UP[ij]{\bdf_k\UP[j]}, \\
%     \label{eq:def_mF_A}
%     &\mFA(i,k,l)=\sum_{j=1}^k\mbA_{l}\UP[ij]{\bdf_k\UP[j]}, \\
%     \label{eq:def_mF_C}
%     &\mFC(i,k,l)=\sum_{j=1}^k\mC_{l}\UP[ij]{\bdf_k\UP[j]}, \\
%     \label{eq:def_mF_L}
%     &\mFL(i,k,l)=\sum_{j=1}^k\mL_{l}\UP[ij]{\bdf_k\UP[j]}. 
% \end{align}
\begin{equation}
    \label{eq:def_mF}
    \begin{split}
        &\mFT(i,k,l)=\sum_{j=1}^k\mT_{l}\UP[ij]{\bdf_k\UP[j]}, \qquad \mFA(i,k,l)=\sum_{j=1}^k\mbA_{l}\UP[ij]{\bdf_k\UP[j]}, \\
        &\mFC(i,k,l)=\sum_{j=1}^k\mC_{l}\UP[ij]{\bdf_k\UP[j]}, \qquad \mFL(i,k,l)=\sum_{j=1}^k\mL_{l}\UP[ij]{\bdf_k\UP[j]}.
    \end{split}
\end{equation}
Some basic facts can be observed:
\begin{enumerate}
    % when $l\geqslant i$, it holds 
    % $$\mFT(i,k,l)=\mFT(i,k,l-1)=\cdots=\mFT(i,k,i-1),$$ 
    % $$\mFA(i,k,l)=\mFA(i,k,l-1)=\cdots=\mFA(i,k,i-1),$$ 
    % $$\mFC(i,k,l)=\mFC(i,k,l-1)=\cdots=\mFC(i,k,i-1),$$
    % $$\mFL(i,k,l)=\mFL(i,k,l-1)=\cdots=\mFL(i,k,i-1).$$
    % Besides, 
    \item When $i>l\geqslant 1$, it holds
    \begin{align}
        \label{eq:rec_l_mFT}
        &\mFT(i,k,l)=\mFT(i,k,l-1)+\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\mFT(l,k,l-1), \\
        \label{eq:rec_l_mFA}
        &\mFA(i,k,l)=\mFA(i,k,l-1)+\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\mFA(l,k,l-1). \\
        \label{eq:rec_l_mFC}
        \begin{split}
            &\mFC(i,k,l)=\mFC(i,k,l-1)+\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\mFC(l,k,l-1)\\
            &\qquad +\pd{}{t}\left[\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\right]\mFT(l,k,l-1)
            +\nabla_{\bx}\left[\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\right]\cdot\mFA(l,k,l-1).
        \end{split}
    \end{align}
    \eqref{eq:rec_l_mFT} and \eqref{eq:rec_l_mFA} can be directly obtained from the definition \eqref{eq:lin_def_TABL_l}. For the third equality, we have 
    \begin{equation}
        \label{eq:exp_C_lij}
        \begin{split}
            \mC\UP[ij]_l=&\pd{}{t}\mT_l\UP[ij]+\nabla_{\bx}\cdot\mbA_l\UP[ij]-\mB_l\UP[ij] \\
            =&\pd{}{t}\left[\mT_{l-1}\UP[ij]+\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\mT_{l-1}\UP[lj]\right]+\nabla_{\bx}\cdot\left[\mbA_{l-1}\UP[ij]+\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\mbA_{l-1}\UP[lj]\right]\\
            &-\left[\mB_{l-1}\UP[ij]+\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\mB_{l-1}\UP[lj]\right] \\
            =&\mC\UP[ij]_{l-1}+\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\mC_{l-1}\UP[lj]+
            \pd{}{t}\left[\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\right]\mT\UP[lj]_{l-1}+\nabla_{\bx}\left[\mL_{l-1}\UP[il]\left(\mL_{l-1}\UP[ll]\right)^{-1}\right]\cdot\mbA\UP[lj]_{l-1}.
        \end{split}
    \end{equation}
    which straightforwardly yields \eqref{eq:rec_l_mFC}. 
    \item from \eqref{eq:exp_T_0ij}, \eqref{eq:exp_A_0ij} and \eqref{eq:exp_C_0ij}, we have
    \begin{align}
        \label{eq:rela_mFTl0}
        &\mFT(i,k,0)=\sum_{l=1}^{i+1}\left(\mT_{l-1}\UP[li]\right)^T\left(\mL_{l-1}\UP[ll]\right)^{-1}\mFL(l,k,l-1), \\
        \label{eq:rela_mFAl0}
        &\mFA(i,k,0)=\sum_{l=1}^{i+1}\left(\mbA_{l-1}\UP[li]\right)^T\left(\mL_{l-1}\UP[ll]\right)^{-1}\mFL(l,k,l-1), \\
        \label{eq:rela_mFCl0}
        &\mFC(i,k,0)=\sum_{l=1}^{i+1}\left(\mB_{l-1}\UP[li]\right)^T\left(\mL_{l-1}\UP[ll]\right)^{-1}\mFL(l,k,l-1). 
    \end{align}
    \item when $k\geqslant 1$, it holds 
    \begin{equation}
        \label{eq:Max_mF}
        \begin{split}
            \mFL(i,k,l)=\Kn\Bigg[&\pd{}{t}\mFT(i,k-1,l)+\nabla_{\bx}\cdot\left(\mbA_l\UP[i0]\bdf\UP[0]\right)+\nabla_{\bx}\cdot\mFA(i,k-1,l)\\
            &+\mC_l\UP[i0]\bdf\UP[0]+\mFC(i,k-1,l)\Bigg],
        \end{split}
    \end{equation}
    which results from the Maxwellian iteration of step $k$ with \eqref{eq:lin_moment_C}.
\end{enumerate}

Now we present the proof of Thm. \ref{thm:linear}.

\begin{proof}[Proof of Thm. \ref{thm:linear}]
Combining \eqref{eq:rela_mFTl0}, \eqref{eq:rela_mFAl0}, \eqref{eq:rela_mFCl0} and \eqref{eq:Max_mF}, it can be obtained that
\begin{equation}
    \label{eq:recur_mFT}
    \begin{split}
        \mFT(i,k,0)=\Kn\sum_{l=1}^{i+1}&\left(\mT_{l-1}\UP[li]\right)^T\left(\mL_{l-1}\UP[ll]\right)^{-1}
        \Bigg[\pd{}{t}\mFT(l,k-1,l-1)+\nabla_{\bx}\cdot\left(\mbA_{l-1}\UP[l0]\bdf\UP[0]\right)\\
        &+\nabla_{\bx}\cdot\mFA(l,k-1,l-1)      
        +\mC_{l-1}\UP[l0]\bdf\UP[0]+\mFC(l,k-1,l-1)\Bigg], 
    \end{split}
\end{equation}
\begin{equation}
    \label{eq:recur_mFA}
    \begin{split}
        \mFA(i,k,0)=\Kn\sum_{l=1}^{i+1}&\left(\mbA_{l-1}\UP[li]\right)^T\left(\mL_{l-1}\UP[ll]\right)^{-1}
        \Bigg[\pd{}{t}\mFT(l,k-1,l-1)+\nabla_{\bx}\cdot\left(\mbA_{l-1}\UP[l0]\bdf\UP[0]\right)\\
        &+\nabla_{\bx}\cdot\mFA(l,k-1,l-1)      
        +\mC_{l-1}\UP[l0]\bdf\UP[0]+\mFC(l,k-1,l-1)\Bigg], 
    \end{split}
\end{equation}
and
\begin{equation}
    \label{eq:recur_mFC}
    \begin{split}
        \mFC(i,k,0)=\Kn\sum_{l=1}^{i+1}&\left(\mB_{l-1}\UP[li]\right)^T\left(\mL_{l-1}\UP[ll]\right)^{-1}
        \Bigg[\pd{}{t}\mFT(l,k-1,l-1)+\nabla_{\bx}\cdot\left(\mbA_{l-1}\UP[l0]\bdf\UP[0]\right)\\
        &+\nabla_{\bx}\cdot\mFA(l,k-1,l-1)      
        +\mC_{l-1}\UP[l0]\bdf\UP[0]+\mFC(l,k-1,l-1)\Bigg].
    \end{split}
\end{equation}

With \eqref{eq:rec_l_mFT}, \eqref{eq:rec_l_mFA} and \eqref{eq:rec_l_mFC}, the right-hand side can be replaced by some summation of $\mFT(i',k-1,0)$, $\mFA(i',k-1,0)$ and $\mFC(i',k-1,0)$, where $i'\leqslant i$. 

The system with approximation order $O(\Kn^{2n})$ can be formulated as
    \begin{equation}
        \label{eq:lin_approx_2n}
        \pd{\bdf\UP[0]}{t}+\mbA_0\UP[00]\cdot \nabla_{\bx}\bdf\UP[0]+\sum_{k=1}^{2n}\mbA_0\UP[0k]\cdot \nabla_{\bx}\bdf_{2n}\UP[k]
        +\mC\UP[00]_0\bdf\UP[0]+\sum_{k=1}^{2n}\mC_0\UP[0k]\bdf_{2n}\UP[k]=0,
    \end{equation}
which can be equivalently expressed by
\begin{equation}
    \label{eq:lin_approx_2n_mF}
    \pd{\bdf\UP[0]}{t}+\mbA_0\UP[00]\cdot \nabla_{\bx}\bdf\UP[0]+\mFA(0,2n,0)+\mC_0\UP[00]\bdf\UP[0]+\mFC(0,2n,0)=0.
\end{equation}

Now we repeatedly use the relationship \eqref{eq:recur_mFT}, \eqref{eq:recur_mFA} and \eqref{eq:recur_mFC} to reduce the second entry of $\mFT$, $\mFA$ and $\mFC$. The process ends while the second entry of all terms reaches $n$. After that, we let the third entry again return to $0$ with \eqref{eq:rec_l_mFT}, \eqref{eq:rec_l_mFA} and \eqref{eq:rec_l_mFC}. 

Ultimately, we can obtain the expressions of $\mFA(0,2n,0)$ and $\mFC(0,2n,0)$, where all the terms of $\mFT, \mFA, \mFC$ have second entry $n$ and the third entry $0$.  
Based on the whole procedure of substitution, some facts can be observed:
\begin{itemize}
    \item During each step in the iteration, the summation of first entry and second entry does not increase. Therefore, in the ultimate expression, the first entry of all terms $\mFT$, $\mFA$ and $\mFC$ are not larger than $n$. Meanwhile, the results of $f_n$ can be accurately computed with $n$ steps of Maxwellian iterations from the truncated moment system \eqref{eq:moment_n}.   
    \item The superscripts of all matrices $\mT, \mbA, \mB, \mL$ involved in the process are not larger than $n$. Thus, they can be directly extracted from \eqref{eq:moment_n}.
\end{itemize}
Consequently, the left-hand side of \eqref{eq:lin_approx_2n} can be precisely obtained from the moment model \eqref{eq:moment_n}, which validates its approximation order of $O(\Kn^{2n})$.   
\end{proof}

\begin{remark}
    From the proof of Thm. \ref{thm:linear}, it can be similarly verified that if one needs the accurate expression of $\mFA(0,2n-1,0)$ and $\mFC(0,2n-1,0)$, the matrices $\mT\UP[nn]$, $\mbA\UP[nn]$ and $\mC\UP[nn]$ are not involved. Hence, these parts could be set as $0$ in the system of approximation order $O(\Kn^{2n-1})$.
\end{remark}


